Fair Allocation of Indivisible Goods: Improvement and Generalization

We study the problem of fair allocation for indivisible goods. We use the the maxmin share paradigm introduced by Budish as a measure for fairness. Procaccia and Wang (EC'14) were first to investigate this fundamental problem in the additive setting. In contrast to what real-world experiments suggest, they show that a maxmin guarantee (1-MMS allocation) is not always possible even when the number of agents is limited to 3. While the existence of an approximation solution (e.g. a $1/2$-MMS allocation) is quite straightforward, improving the guarantee becomes subtler for larger constants. Procaccia provide a proof for existence of a $2/3$-MMS allocation and leave the question open for better guarantees. Our main contribution is an answer to the above question. We improve the result of [Procaccia and Wang] to a $3/4$ factor in the additive setting. The main idea for our $3/4$-MMS allocation method is clustering the agents. To this end, we introduce three notions and techniques, namely reducibility, matching allocation, and cycle-envy-freeness, and prove the approximation guarantee of our algorithm via non-trivial applications of these techniques. Our analysis involves coloring and double counting arguments that might be of independent interest. One major shortcoming of the current studies on fair allocation is the additivity assumption on the valuations. We alleviate this by extending our results to the case of submodular, fractionally subadditive, and subadditive settings. More precisely, we give constant approximation guarantees for submodular and XOS agents, and a logarithmic approximation for the case of subadditive agents. Furthermore, we complement our results by providing close upper bounds for each class of valuation functions. Finally, we present algorithms to find such allocations for additive, submodular, and XOS settings in polynomial time.

==> acknowledgement.tex <==
\section{Acknowledgment}
We would like to thank Alireza Farhadi for having very helpful discussions.

==> conc.tex <==
\section{Conclusion}
We have studied the problem of allocating items to the players, and tried to guarantee an approximation of maxmin-share for each player. We gave a $\frac{4}{5}$-MMS allocation algorithm for $n=4$. One future work would be improving this approximations for general $n$ or special cases like $n=3,4$ , or giving an upper bound on the maximum possible value of $\alpha$ for any $\alpha$-MMS allocation. 

For general $n$, we provided a new $\frac{2}{3}$-MMS algorithm with less dependency to the definition of MMS and proved that regarding the \emph{weak linearity} condition, the algorithm can be turn into a $\frac{2}{3}$ proportional allocation. An extension here is to exactly determine how likely is it for an instance of a problem to satisfy \emph{weak linearity}, e.g. when the value of items are chosen uniformly from $[0,1]$. With the same deduction as Lemma 1 for proportionality, we can assume that all the items have values less than $\frac{2}{3}$. Regarding this fact, we think it is common for a set of items to preserve \emph{weak linearity} condition.

Another direction is extending the algorithm for more general valuations functions such as submodular valuations. In that case, using the queries mentioned in Section 3 to implement the algorithm would be much more convincing.

Finally, generalizing our method for classification of the players and items may help to give better approximation ratio than $\frac{2}{3}$. 

==> defend.tex <==
%\section{A Note for The Reviewers}\label{defend}
We received some controversial critiques, among many positive comments, from FOCS'16 that we would like to respond to.
 \textit{''The complexity of the algorithm was seen as a minus and it was hard to get any new insights from it''}: such comments are very rarely (if ever) given especially in venues such as FOCS and STOC. Of course the solution is not trivial, nonetheless we do not believe it is fair to see this as a minus for a paper. In Section \ref{overview}, we clearly outline the algorithm, how it has been derived from previous works, and how it can be further improved to achieve better bounds.
 With regard to the presentation, we would like to note that we received positive feedback on an earlier version of the paper submitted to FOCS'16: \textit{''Although it is very complex, the authors make a good job in explaining the ideas and I like them."}. However, we further improved the presentation style (abstract, intro, and technical parts), based on the comments we received from other reviewers.
 Following on a comment on the applicability of our algorithms, we would like to note that our algorithms are efficient and easy to implement. What makes the paper slightly hard to understand is the analysis of the algorithms. You can find an implemented version of the algorithms at \href{}{text}.

